Embracing Error to Enable Rapid Crowdsourcing

Microtask crowdsourcing has enabled dataset advances in social science and machine learning, but existing crowdsourcing schemes are too expensive to scale up with the expanding volume of data. To scale and widen the applicability of crowdsourcing, we present a technique that produces extremely rapid judgments for binary and categorical labels. Rather than punishing all errors, which causes workers to proceed slowly and deliberately, our technique speeds up workers' judgments to the point where errors are acceptable and even expected. We demonstrate that it is possible to rectify these errors by randomizing task order and modeling response latency. We evaluate our technique on a breadth of common labeling tasks such as image verification, word similarity, sentiment analysis and topic classification. Where prior work typically achieves a 0.25x to 1x speedup over fixed majority vote, our approach often achieves an order of magnitude (10x) speedup.

==> RSVP (1)/intro_v6.tex <==
Social science~\cite{kittur2008crowdsourcing, mason2012conducting}, interactive systems~\cite{fast2014emergent, kumar2013webzeitgeist} and machine learning~\cite{deng2009imagenet, lin2014microsoft} are becoming more and more reliant on large-scale, human-annotated data. Increasingly large annotated datasets have unlocked a string of social scientific insights~\cite{gilbert2009predicting, burke2013using} and machine learning performance improvements~\cite{krizhevsky2012imagenet, girshick2014rich, vinyals2014show}. One of the main enablers of this growth has been microtask crowdsourcing~\cite{snow2008cheap}. Microtask crowdsourcing marketplaces such as Amazon Mechanical Turk offer a scale and cost that makes such annotation feasible. As a result, companies are now using crowd work to complete hundreds of thousands of tasks per day~\cite{marcuswaran}.

However, even microtask crowdsourcing can be insufficiently scalable, and it remains too expensive for use in the production of many industry-size datasets~\cite{josephy2013crowdscale}. Cost is bound to the amount of work completed per minute of effort, and existing techniques for speeding up labeling (reducing the amount of required effort) are not scaling as quickly as the volume of data we are now producing that must be labeled~\cite{thomee2016yfcc100m}. To expand the applicability of crowdsourcing, %understand and keep up with the ever-expanding stream of data, 
the number of items annotated per minute of effort needs to increase substantially.

\begin{figure*}
  \centering
  \includegraphics[width=2\columnwidth]{figures/pull_figure.png}
  \caption{(a) Images are shown to workers at 100ms per image. Workers react whenever they see a dog. (b) The true labels are the ground truth dog images. (c) The workers' keypresses are slow and occur several images after the dog images have already passed. We record these keypresses as the observed labels. (d) Our technique models each keypress as a delayed Gaussian to predict (e) the probability of an image containing a dog from these observed labels.}
  %These learned likelihoods are then used to annotate all the images that contain a dog.}
  \label{fig:pull_figure}
\end{figure*}

In this paper, we focus on one of the most common classes of crowdsourcing tasks \cite{ipeirotis2010analyzing}: binary annotation. These tasks are yes-or-no questions, typically identifying whether or not an input has a specific characteristic. Examples of these types of tasks are topic categorization (e.g., ``Is this article about finance?'')~\cite{schapire2000boostexter}, image classification (e.g., ``Is this a dog?'')~\cite{deng2009imagenet, lin2014microsoft, li2003detecting}, audio styles~\cite{seetharaman2014crowdsourcing} and emotion detection~\cite{li2003detecting} in songs (e.g., ``Is the music calm and soothing?''), word similarity (e.g., ``Are \textit{shipment} and \textit{cargo} synonyms?'')~\cite{miller1991contextual} and sentiment analysis (e.g.,\ ``Is this tweet positive?'')~\cite{pang2008opinion}. 

%where previous crowdsourcing work seeks to minimize and recover from error, we seek to encourage it. *Encouraging* crowd workers to make mistakes,  and even designing the task to make mistakes inevitable, produces far greater speedups than recovering from error posthoc.

Previous methods have sped up binary classification tasks by minimizing worker error.
%reducing the number of workers needed to achieve high accuracy. 
A central assumption behind this prior work has been that workers make errors because they are not trying hard enough (e.g.,\ ``a lack of expertise, dedication [or] interest''~\cite{sheng2008get}).
Platforms thus punish errors harshly, for example by denying payment. Current methods calculate the minimum redundancy necessary to be confident that errors have been removed~\cite{sheng2008get, smyth1994knowledge, smyth1995inferring}. These methods typically result in a 0.25$\times$ to 1$\times$ speedup beyond a fixed majority vote~\cite{peng2010decision,russakovsky2015best,sheng2008get,karger2014budget}.

We take the opposite position: that designing the task to encourage some error, or even make errors inevitable, can produce far greater speedups.
%The main challenge is not that workers are not trying hard enough, but that they are trying \emph{too hard}. 
Because platforms strongly punish errors, workers carefully examine even straightforward tasks to make sure they do not represent edge cases~\cite{martin2014being, irani2013turkopticon}. The result is slow, deliberate work. 
We suggest that there are cases where we can encourage workers to move quickly by telling them that making some errors is acceptable.
%We suggest that there are cases where it is more effective to tell workers that making some errors is acceptable, and then encourage them to move quickly. 
Though individual worker accuracy decreases, we can recover from these mistakes post-hoc algorithmically (Figure~\ref{fig:pull_figure}).

We manifest this idea via a crowdsourcing technique in which workers label a rapidly advancing stream of inputs. Workers are given a binary question to answer, and they observe as the stream automatically advances via a method inspired by rapid serial visual presentation (RSVP)~\cite{li2002rapid, fei2007we}. Workers press a key whenever the answer is ``yes'' for one of the stream items. Because the stream is advancing rapidly, workers miss some items and have delayed responses. However, workers are reassured that the requester expects them to miss a few items. To recover the correct answers, the technique randomizes the item order for each worker and model workers' delays as a normal distribution whose variance depends on the stream's speed. For example, when labeling whether images have a ``barking dog'' in them, a self-paced worker on this task takes 1.7s per image on average. With our technique, workers are shown a stream at 100ms per image. The technique models the delays experienced at different input speeds and estimates the probability of intended labels from the key presses.

We evaluate our technique by comparing the total worker time necessary to achieve the same precision on an image labeling task as a standard setup with majority vote.
%on an image labeling task by comparing it to the total a conventional binary labeling interface %in which workers work at their own pace and try not to make errors. We compare the total worker time necessary to achieve the same precision as a standard setup of three workers decided via majority vote (1.7s each). 
The standard approach takes three workers an average of 1.7s each for a total of 5.1s.
Our technique achieves identical precision (97\%) with five workers at 100ms each, for a total of 500ms of work. The result is an order of magnitude speedup of 10$\times$. %Our approach is able to label images with precision of 97\%. 

This relative improvement is robust across both simple tasks, such as identifying dogs, and complicated tasks, such as identifying ``a person riding a motorcycle'' (interactions between two objects) or ``people eating breakfast'' (understanding relationships among many objects). We generalize our technique to other tasks such as word similarity detection, topic classification and sentiment analysis. Additionally, we extend our method to categorical classification tasks through a ranked cascade of binary classifications. Finally, we test workers' subjective mental workload and find no measurable increase.
% Finally, we test workers' subjective mental workload and find that our technique does not measurably increase it.
%demonstrate how our technique can be combined with existing crowdsourcing methods to annotate a subset of a popular image dataset with a speedup of $50\times$.

\textbf{Contributions}. We make the following contributions:
\begin{enumerate}
  \setlength{\itemsep}{1pt}
%  \setlength{\parskip}{0pt}
%  \setlength{\parsep}{0pt}
\item We introduce a rapid crowdsourcing technique that makes errors normal and even inevitable. We show that it can be used to effectively label large datasets by achieving a speedup of an order of magnitude on several binary labeling crowdsourcing tasks.
\item We demonstrate that our technique can be generalized to multi-label categorical labeling tasks, combined independently with existing optimization techniques, and deployed without increasing worker mental workload.
\end{enumerate}
